Semantically Enhanced Software Traceability Using Deep Learning Techniques

In most safety-critical domains the need for traceability is prescribed by certifying bodies. Trace links are generally created among requirements, design, source code, test cases and other artifacts, however, creating such links manually is time consuming and error prone. Automated solutions use information retrieval and machine learning techniques to generate trace links, however, current techniques fail to understand semantics of the software artifacts or to integrate domain knowledge into the tracing process and therefore tend to deliver imprecise and inaccurate results. In this paper, we present a solution that uses deep learning to incorporate requirements artifact semantics and domain knowledge into the tracing solution. We propose a tracing network architecture that utilizes Word Embedding and Recurrent Neural Network (RNN) models to generate trace links. Word embedding learns word vectors that represent knowledge of the domain corpus and RNN uses these word vectors to learn the sentence semantics of requirements artifacts. We trained 360 different configurations of the tracing network using existing trace links in the Positive Train Control domain and identified the Bidirectional Gated Recurrent Unit (BI-GRU) as the best model for the tracing task. BI-GRU significantly out-performed state-of-the-art tracing methods including the Vector Space Model and Latent Semantic Indexing.

==> ResultsNew.tex <==
\section{Results and Discussion}
\label{sec:result}
%Using the experiment setting described in Section \ref{sec:experiment}, we aim to explore whether different configurations of the tracing network perform differently in term of minimizing the loss on development dataset, if so, what is the best configuration and whether the tracing network using this configuration can achieve better tracing result than other tracing methods.
In this section, we report (1) the best configurations found in our network configuration search space, (2) the performance of the tracing network with the best configuration compared against VSM and LSI, and (3) the performance of the tracing network when trained with a larger training set of data. 

\subsection{What is the best configuration for tracing network?}
\label{subsec:exp1}

This experiment aims to address the first research question (RQ1). When optimizing the network configuration of the tracing network, we first selected the best configuration for each RNN unit type; Table \ref{tab:BestHyperparamPerModel} summarizes these results. We found that the best configurations for all four RNN unit types were very similar: one layer RNN model with 30 hidden dimensions and a Integration layer of 10 hidden dimensions, learning rate of 1e-02, gradient clip value of 10, and $\lambda$ of 1e-04. But for different RNN unit type, the performance varies.

\begin{table}[h]
  \caption{Best Configuration for Each RNN Unit Type}
  \label{tab:BestHyperparamPerModel}
    \begin{center}
        \begin{tabular}{p{1.2cm}p{0.6cm}p{1cm}llllll}
            \toprule
            \thead{RNN\\Unit} & \thead{Dev.\\Loss} & \thead{Word\\Emb.} & \thead{$L$} & \thead{$D_r$} & \thead{$D_s$} & \thead{$lr$} & \thead{$gc$} & \thead{$\lambda$}\\
            \midrule
            %\textbf{RNN Unit}&\textbf{Dev. Loss}&\textbf{Word Emb.}&\textbf{$L$}&\textbf{$D_r$}&\textbf{$D_s$}&\textbf{$lr$}&\textbf{$gc$}&\textbf{$\lambda$}\\} \hline
            BI-GRU  & .1045     & PTC       &1    & 30   & 10 & .01  & 10      & .0001 \\
            GRU     & .1301     & PTC       &1    & 30   & 10 & .01  & 10      & .0001 \\
            BI-LSTM & .1434     & PTC       &1    & 30   & 10 & .01  & 100     & .0001 \\
            LSTM    & .2041     & PTC+Wiki  &1    & 30   & 10 & .01  & 10      & .0001 \\
            \bottomrule
            %AveVect  & 0.2775           & PTC       &/    & /   & 10 & 0.01  & /     & 0.0001 \\ \hline
        \multicolumn{9}{p{8.5cm}}{$L$ -- number of layers in the RNN model, $D_r$ -- hidden dimension in RNN unit, $D_s$ -- hidden dimension in Integration layer, $lr$ -- initial learning rate, $gc$ -- gradient clipping value, $\lambda$ -- regularization strength}
        \end{tabular}
    \end{center}
    \vspace{-12pt}
\end{table}

Figure \ref{fig:learningCurve} illustrates the learning curves on the training dataset of the four configurations. All four RNN unit types outperformed the Average Vector method. This supports our hypothesis that word order plays an important role when comparing the semantics of sentences. Both GRU and BI-GRU achieved faster convergence and more desirable (smaller) loss than LSTM and BI-LSTM. Although quite similar, the bidirectional models performed slightly better than the unidirectional models for both GRU and LSTM on the training set; the bidirectional models also achieved better results on the development dataset compared to their unidirectional counterparts. As a result, the overall best performance was achieved using \textbf{BI-GRU} configured as shown in Table \ref{tab:BestHyperparamPerModel}.

\begin{figure}[h]
\centering
\includegraphics[width=0.49\textwidth]{figures/ModelComparison.pdf}
\caption{Comparison of learning curves for each RNN variant using its best configuration. GRU and BI-GRU converse faster and achieved smaller loss than LSTM, BI-LSTM, and baseline.}
\label{fig:learningCurve}
\vspace{-4pt}
\end{figure}

We also found that in three of the four best configurations, the word embedding vectors were trained using the PTC corpus alone. We speculate that one reason the PTC-trained word vectors performed better than the PTC+Wiki-trained vectors is due to differences in content of the two corpora. The PTC+Wiki corpus contains significantly more words that are used in diverse contexts because the majority of articles in the Wiki corpus are not related to the PTC domain. In the case of words that appear commonly in Wiki articles but convey specific meanings in the PTC domain (e.g. message, administrator, field, etc.), their context in the general articles is likely to negatively affect the reasoning task on domain specific semantics when there is insufficient training data to disambiguate their usage. We also tested the tracing network performance using 300-dimension word embedding trained by PTC corpus. The result is similar to the best configuration we find in Table \ref{tab:BestHyperparamPerModel}. These findings suggest that using only the domain corpus to train word vectors with a reasonable size is more computationally economic and can yield better results.


%There might be two reasons that using the word vectors trained by PTC corpus out-performs using the word vectors trained by PTC+Wiki corpus. Because it contains more parameters in the tracing network to use the 300 dimension word vectors, it is harder to train. Therefore, the first explanation is that we didn't train the tracing network with 300 dimension word vectors well enough with the configuration setting and training dataset. The second explanation could be due to the difference in the content of the two sets of word vectors. Vectors that are trained by PTC+Wiki corpus contains significantly more words and words used in different context. The majority of articles in Wiki dump are not related to the PTC domain. For many words that appear commonly in Wiki articles but convey specific meanings in PTC domain, their context in the general articles might negatively affect the reasoning task on domain specific semantics when the tracing model is not complex enough to differentiate the uasage. To shed some light on which explanation is more plausible, we conduct an additional experiment that re-train the tracing network with the best configuration that used 300 dimension word vectors, but we switch word vectors trained by PTC+Wiki corpus to 300 dimensional word vectors trained by PTC corpus. The result is shown in Table \ref{tab:wordVectorSource}. The minimum loss on development set decreases from 0.1584 to 0.1084. This is comparable to the best configuration we find in Table \ref{tab:BestHyperparamPerModel}. We therefore believe that the different performance is more likely due to the difference in the content of word vectors than the dimensions. Notice that using PTC corpus but increase the dimension of word vectors from 50 to 300 doesn't imporove the network performance. We conclude that using the domain corpus to train word vectors with reasonable size is more computationally economical and yield better result.

% \begin{table}
%   \caption{Comparing Minimum loss on development datasets using Word Vectors trained by PTC and PTC+Wiki corpus}
%   \label{tab:wordVectorSource}
%     \begin{center}
%         \begin{tabular}{|l|l|l|l|}\hline
%             Word Emb. Source & PTC+Wiki, 300d & PTC, 300d & PTC, 50d\\ \hline
%             Min Dev Loss  & 0.1584 &  0.1084  & 0.1045 \\ \hline
%         \end{tabular}
%     \end{center}
% \end{table}



\subsection{Does the tracing network outperform leading trace retrieval algorithms?}
\label{subsec:exp2}
We now evaluate whether the best configuration of the tracing network (i.e. BI-GRU with configuration shown in Table \ref{tab:BestHyperparamPerModel}) outperforms leading trace retrieval algorithms, we used it to generate link probabilities for each  source and target artifact pair in the test set (45\% total data). For each source artifact, the generated links were ranked by descending probability scores and Average Precision ($AP$) was calculated using Equation \ref{eq:AvgPrec}. We then compared the APs associated with our tracing network with those generated using the best performing VSM and LSI configurations. Our tracing network was able to achieve a MAP of .598; this value is 41\% higher than that achieved using VSM (\emph{MAP} = .423) and 32\% higher than LSI (\emph{MAP} = .451). We conducted a Kruskal-Wallis test and found a statistically significant difference among the AP values associated with the three methods ($H(2)=91.36$, $p<.001$). We then conducted three pairwise Mann-Whitney U tests with Bonferroni p-value adjustments. Results indicated that the APs associated with our tracing network were significantly higher (\emph{M} = .598, \emph{SD} = .370) than those achieved using VSM (\emph{M} = .423, \emph{SD} = .391; $p<.001$) and LSI (\emph{M} = .451, \emph{SD} = .400; $p<.001$); in contrast, there was no significant difference when comparing APs for VSM versus those for LSI.

When comparing the Precision-Recall Curves for the three methods (Figure \ref{fig:prCurve_45_45_10}), we observed that the tracing network outperformed VSM and LSI at higher levels of recall. Given the goal to achieve close to 100\% recall when performing tracing tasks, this is an important achievement. Precision improved notably when recall was above 0.2. This improvement can be attributed to the fact that the tracing network is able to extract semantic information from artifacts and to reason over associations between them. While it is almost impossible to completely decipher how GRU extracts a semantic vector from natural language \cite{DBLP:journals/corr/KarpathyJL15}, observing gate behavior when GRU processes a sentence can provide some insights into how GRU performs this task so well.
%Jane:Has anyone tried this before? 
%Jin:There's some, but not the way we did it in this paper
As an example, we examine the gate behavior when our best performing GRU processes the following artifact text: \textit{``Exceptions: If the SA\_FileTransferConfiguration datapoint indicates that the BOS is not configured for file transfer, the File Transfer Manager sends an 01105\_FileTransferUnavailable message to the On\-board.''}.

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/PRCurve_45_45_10.pdf}
\caption{Precision-Recall Curve on test set -- 45\% total data}
\label{fig:prCurve_45_45_10}
\end{figure}

The gate behavior varies among dimensions in the sentence semantic vector. In Figure \ref{fig:gateOutput}, we show the levels of the reset and the update gates and the change of the output values on two of the 30 dimensions after GRU takes each word from this artifact. %Recall that the \textbf{update gate} decides how much the unit updates its output based on its current input; when the update gate is small, the unit simply preserves its previous ``memory'' and ignores the current input. In contrast, the \textbf{reset gate} determines how much previous ``memory'' should be forgotten when it takes the current input. -- not really true -- they work together -- hard to decouple
Unlike LSTM, the GRU does not have an explicit memory cell; however, the unit output itself can be considered as a \emph{persisting memory} while the output candidate in Equation \ref{eq:gru_h_cand} acts as a \emph{temporary memory}. Recall that the \textbf{reset gate} controls how much previous output adds to the current input when determining the output candidate (i.e. temporary memory); in contrast, the \textbf{update gate} balances the contributions of this temporary memory and the previous output  (i.e. persisting memory) to the actual current output. From Figure \ref{fig:gateBehavior}, we observe that for the 24th dimension, the reset gate is constantly small. This means that the temporary memory is mostly decided by the current input word. The update gate for this dimension was also small for most of the input words until the words \textit{datapoint},  \textit{transfer} and \textit{to} came. Those spikes indicate moments when the temporary memory was integrated into the persisting memory. As such, we can speculate that this semantic vector dimension functions to accumulate  information from specific keywords across the entire sentence. Conversely, for the 12th dimension, the reset gate was constantly high, indicating that the information stored in the temporary memory was based on both previous output and current input. Therefore, the actual output is more sensitive to local context rather than a single keyword. This is confirmed by the fluctuating shape of the actual output shown in the figure. For example, the output value remained in the same range until the topic was changed from ``datapoint indication'' to ``message transfer''. We believe that this versatile behavior of the gating mechanism might enable GRU to encode complex semantic information from a sentence into a vector to support trace link generation and other challenging NLP tasks.  
%Jane:ANY supporting refs for this type of analysis?? 
%Jin:I haven't seen any similar analysis. I've weakened the conclusion 

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[width=\textwidth]{figures/GateOutputInstruct.pdf}
        \caption{GRU output at one time step}
        \label{fig:snippet}
    \end{subfigure}
    
    \vspace{0.3cm}

    
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/GateOutput.pdf}
        \caption{GRU gate behavior}
        \label{fig:gateBehavior}
    \end{subfigure}

    \caption{The reset gate and update gate behavior in GRU and their corresponding output on the 24th and 12th dimension of sentence semantic vector. The x-axis indicates the sequential input of words while the y-axis is the value of reset gate, update gate and output after taking each word.}\label{fig:gateOutput}
    \vspace{-16pt}
\end{figure}

From Figure \ref{fig:prCurve_45_45_10}, we also notice that the tracing network hits a glass ceiling for improving precision above 0.27. We consider this to be caused by its inability to rule out some false positive links that contain valid associations. For example, the tracing network assigns a 97.27\% probability of a valid link between artifact \textit{``The BOS administrative toolset shall allow an authorized administrator to view internal errors generated by the BOS''} and the artifact \textit{``The MessagesEvents panel provides the functionality to view message and event logs.  The panel provides searching and filtering capabilities where the user can search by a number of parameters depending on the type of data the user wants to view.''}. There are direct associations between these artifacts: MessagesEvents panel is part of the BOS administrative toolset for viewing message and event log, administrator is a system user and internal errors generated by the BOS is an event. But this is not a valid link because MessagesEvents panel only displays messages and events related to external Railroad Systems rather than to internal events. It is likely that the tracing network fails to exclude this link because it has not been exposed to sufficient similar negative examples in the training data. As we described in Section \ref{subsec:dataPreparation}, every positive example is used while negative examples (i.e. non-links) are randomly selected during each epoch. We plan to explore more adequate methods for handling unbalanced data problems caused by characteristics of the tracing data in our future work.


\subsection{How does the tracing network react to more training data?}
\label{subsec:exp3}
As a software project proceeds, an increasing number of trace links are often created. To explore the potential impact of folding them into the training set, we increased the portion of the training dataset to 80\%. Specifically, we randomly selected part of the test data and moved it into the training set to reach 80\%. The remaining data was retained in the testing set. Using the same configuration as described in Section \ref{subsec:networkOptimization}, we then retrained the tracing network. Because the size of the test set decreased to 10\%, we could not make direct comparisons to our previous results.  Instead we used both of the trained tracing networks (i.e. trained with 45\% and 80\% of the data respectively) to generate trace links against the same small test set (sized at 10\%).


%We then retrained the tracing netWe re-train the tracing network configured in the same way as the experiment described in Section \ref{subsec:networkOptimization}. We compared the result obtained with this new data division with that of our original tracing model on the same testing set (10\% of total dataset).
%Note that when the testing dataset is smaller, the possible links to return for each query is shorter thus would yield higher MAP in general. To eliminate this effect, the result of our is the result on the same testing data (10\% of total dataset).

With larger sized training set, the \emph{MAP} was .824 compared to .779 for the smaller sized training set.  Results are  depicted in the Precision-Recall Curve in Figure \ref{fig:PRCurve_before_after}. With increased training data, the network can better differentiate links and non-links, and therefore improve both precision and recall. The greatest improvements were observed at lower levels of recall. 

% This suggested that the minimum development loss does not improve because this model represents the best configuration that are not over-trained given a relatively smaller training set (45\%) \hilight{A bit confusing}. The regularization part in the objective function \ref{eq:loss} sets the limit for the minimum loss the network can achieve given specific network configuration. Even so, the tracing accuracy still benefits from using more training data. The MAP using tracing network increases from .598 to .829. \hilight{But we expect this because data set is smaller}.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figures/PRCurve_before_after.pdf}
\caption{Precision-Recall Curve on test set -- 10\% total data.}
\label{fig:PRCurve_before_after}
\end{figure}

The performance of our tracing network was again compared against VSM and LSI for this larger training set. A Kruskal-Wallis test identified a statistically significant difference among the APs associated with the three methods on this new dataset division ($H(2)=19.723.87$, $p<.001$). Using pairwise Mann-Whitney U tests with Bonferroni p-value adjustments, we found that our tracing network performed significantly better (\textbf{\emph{MAP} = .824}) than VSM (\textbf{\emph{MAP} = .612}; $p<.001$) and LSI (\textbf{\emph{MAP} = .704}; $p=0.036$); there was no significant difference between the performance of VSM and LSI on this new data setting. 
Consequently, we can address RQ2 and conclude that our tracing network  improved trace link accuracy in comparison to both VSM and LSI -- both are state-of-the-art techniques for generating trace links. In future work we expect additional improvements by reconfiguring the tracing network for use with a larger training set \cite{bengio2012practical}.

%To the best of our knowledge, no other fully automated techniques have been shown to consistently outperform VSM and LSI.

%Additionally, we think there is space to further improve the performance of the tracing network with more training data. The configuration of this model is optimized for a training set with 45\% of total data. When the training dataset increases, more data points would allow a more complex model to be trained without overfitting leading to more significant improvements in performance \cite{bengio2012practical}. We will explore how we should change our model configuration for best performance for this dataset division in our future work.

